SEA: Evaluating Sketch Abstraction Efficiency via Element-level Commonsense Visual Question Answering

A sketch is a distilled form of visual abstraction that conveys core concepts through simplified yet purposeful strokes while omitting extraneous detail. Despite its expressive power, quantifying the efficiency of semantic abstraction in sketches remains challenging. Existing evaluation methods that rely on reference images, low-level visual features, or recognition accuracy do not capture abstraction, the defining property of sketches. To address these limitations, we introduce SEA (Sketch Evaluation metric for Abstraction efficiency), a reference-free metric that assesses how economically a sketch represents class-defining visual elements while preserving semantic recognizability. These elements are derived per class from commonsense knowledge about features typically depicted in sketches. SEA leverages a visual question answering model to determine the presence of each element and returns a quantitative score that reflects semantic retention under visual economy. To support this metric, we present CommonSketch, the first semantically annotated sketch dataset, comprising 23,100 human-drawn sketches across 300 classes, each paired with a caption and element-level annotations. Experiments show that SEA aligns closely with human judgments and reliably discriminates levels of abstraction efficiency, while CommonSketch serves as a benchmark providing systematic evaluation of element-level sketch understanding across various vision-language models.

==> fig/suppl_oss/commonsketch_clip_1.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=0.99\linewidth]
{fig/suppl_oss/combine1_CLIP_montage.png}
\caption{\textbf{Qualitative examples by SEA score on CommonSketch (set 1).}
Seven CommonSketch classes are shown (\texttt{airplane}, \texttt{basket}, \texttt{bed}, \texttt{bridge},
\texttt{cactus}, \texttt{camera}, \texttt{cat}).
All sketches display four SEA variants computed under different commonsense databases and annotators:
\emph{GPT4o} (GPT-4o database + GPT-4o annotations),
\emph{GPT4o\_OSS} (GPT-OSS database + GPT-4o annotations),
\emph{Qwen} (GPT-4o database + Qwen annotations),
and \emph{Qwen\_OSS} (GPT-OSS database + Qwen annotations).}
\label{fig:commonsketch_clip1}
\end{figure}

==> fig/suppl_oss/commonsketch_clip_2.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=0.99\linewidth]
{fig/suppl_oss/combine2_CLIP_montage.png}
\caption{\textbf{Qualitative examples by SEA score on CommonSketch (set 2).}
Seven additional CommonSketch classes are shown (\texttt{dragon}, \texttt{ear}, \texttt{guitar},
\texttt{helmet}, \texttt{pizza}, \texttt{scissors}, \texttt{sock}).
All sketches display four SEA variants computed under different commonsense databases and annotators:
\emph{GPT4o} (GPT-4o database + GPT-4o annotations),
\emph{GPT4o\_OSS} (GPT-OSS database + GPT-4o annotations),
\emph{Qwen} (GPT-4o database + Qwen annotations),
and \emph{Qwen\_OSS} (GPT-OSS database + Qwen annotations).}
\label{fig:commonsketch_clip2}
\end{figure}

==> fig/suppl_oss/seva_6classes.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=0.99\linewidth]
{fig/suppl_oss/combined_CLIP_montage.png}
\caption{\textbf{Qualitative examples by SEA score on SEVA.}
Six SEVA classes are shown (\texttt{baseball}, \texttt{butterfly}, \texttt{giraffe}, \texttt{guitar}, \texttt{hat}, \texttt{snail}),
with eight sketches per class selected to span a low-to-high SEA range for visual inspection.
All sketches display four SEA variants computed under different commonsense databases and annotators:
\emph{GPT4o} (GPT-4o database + GPT-4o annotations),
\emph{GPT4o\_OSS} (GPT-OSS database + GPT-4o annotations),
\emph{Qwen} (GPT-4o database + Qwen annotations),
and \emph{Qwen\_OSS} (GPT-OSS database + Qwen annotations).}
\label{fig:seva_6classes}
\end{figure}

==> fig/suppl_reward/item.tex <==
\begin{figure}[t]
\centering
% Row 1: Over-detail (g on/off)
\begin{subfigure}[t]{0.4\linewidth}
  \centering
  \includegraphics[width=\linewidth]{z_fig/reward_term/duck_67.png}
  \caption{Over-detail}
  \label{fig:overdetail}
\end{subfigure}
\hfill
% Row 1: Low-recog (g on/off)
\begin{subfigure}[t]{0.4\linewidth}
  \centering
  \includegraphics[width=\linewidth]{z_fig/reward_term/airplane_20.png}
  \caption{Low-recognizability}
  \label{fig:lowrecog}
\end{subfigure}

% Row 2: Table (inside figure)
\begin{subfigure}[t]{0.98\linewidth}
\centering
\scriptsize
\setlength{\tabcolsep}{3pt}
\renewcommand{\arraystretch}{0.9}
\begin{tabular}{lcccc}
\toprule
 & $v{=}V/E$ & $P$ & SEA (w/ $g$) & SEA (w/o $g$) \\
\midrule
Over-detail & 0.692 & 0.631 & -0.428 & +0.168 \\
Low-recog.  & 0.600 & 0.178 & -0.925 & +0.027 \\
\bottomrule
\end{tabular}
\caption{Numerical summary of the two examples.}
\label{fig:example_table}
\end{subfigure}
\vspace{-3pt}
\caption{Qualitative examples illustrating the role of the centered gate $g(\cdot)$. 
When $v>P$, $g(\cdot)<0$ suppresses SEA; removing $g(\cdot)$ yields misleadingly higher scores.}
\label{fig:gate_examples}
\end{figure}


==> fig/userstudy/Reanalysis_outlier.tex <==
\begin{figure}
\centering
\includegraphics[width=0.95\linewidth]{fig/userstudy/Reanalysis_outlier.pdf}
\caption{\textbf{Comparison of human abstraction score distributions and SEA metric scores} for the nose, leaf, and angel classes. Outlier samples in each class are annotated with their SEA scores and mean human abstraction scores.}
\label{jaeyoonoutlier}
\end{figure}

==> fig/userstudy/clip_human_model.tex <==
\begin{figure}
\centering
\includegraphics[width=0.95\linewidth]{fig/userstudy/clip_human_model.png}
\caption{Comparison between human accuracy (H) and the model’s predicted probability (M).}
\label{jaeyoonclassification}
\end{figure}

==> tbl/300_class/item.tex <==
\begin{table*}[t]
\centering
\small
\setlength{\tabcolsep}{5pt}
\begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}llllllllll@{}}
bread & hamburger & hot\_dog & noodle & pizza & pretzel & sandwich & asparagus & broccoli & carrot \\
garlic & mushroom & onion & peanut & pumpkin & apple & banana & grapes & pear & pineapple \\
strawberry & watermelon & cake & cookie & cupcake & donut & ice\_cream\_cone & lollipop & alpaca & boar \\
camel & cat & chameleon & cow & crab & crocodile & deer & dog & dolphin & elephant \\
fish & frog & giraffe & hedgehog & hippopotamus & horse & jellyfish & kangaroo & koala & lion \\
lobster & monkey & moose & octopus & panda & rabbit & seahorse & shark & sheep & sloth \\
snail & snake & squirrel & tiger & turtle & whale & zebra & bat & mole & squid \\
mouse & bird & duck & goose & owl & parrot & peacock & penguin & rooster & swan \\
flamingo & feather & ant & bee & butterfly & dragonfly & caterpillar & scorpion & spider & t-shirt \\
sock & shoe & flip\_flops & belt & bowtie & hat & crown & broom & compass & drill \\
hammer & saw & scissors & screwdriver & shovel & key & ladder & rake & matches & pipe \\
umbrella & binoculars & lighter & mug & wine glass & bottle cap & tent & axe & cannon & grenade \\
rifle & sword & boomerang & fork & spoon & frying\_pan & teapot & knife & bandage & stethoscope \\
syringe & comb & toothbrush & toothpaste & baseball & baseball\_bat & basketball & golf\_club & soccer\_ball & table\_tennis \\
tennis\_racquet & skateboard & roller\_skate & helmet & barbell & dumbbell & parachute & snorkel & ambulance & bicycle \\
bulldozer & bus & car & cruise\_ship & motorcycle & pickup\_truck & train & truck & van & airplane \\
blimp & canoe & helicopter & hot\_air\_balloon & rocket & sailboat & space\_shuttle & submarine & tractor & flying\_saucer \\
wheel & cello & clarinet & drums & guitar & harp & piano & saxophone & trombone & trumpet \\
violin & bell & ear & eye & foot & hand & mouth & nose & tooth & backpack \\
basket & bucket & envelope & mailbox & present & purse & suitcase & wine\_bottle & bed & couch \\
drawer & table & toilet & bathtub & door & stairs & book & calendar & map & marker \\
paper\_clip & paintbrush & pencil & crayon & candle & ceiling\_fan & chandelier & floor\_lamp & lantern & light\_bulb \\
fireplace & hourglass & vase & calculator & camera & charger & computer & keyboard & laptop & alarm\_clock \\
cell\_phone & headphones & megaphone & microphone & radio & satellite & telephone & television & ipod & walkie\_talkie \\
fan & robot & microwave & oven & toaster & bamboo & cactus & clover & dandelion & flower \\
leaf & palm\_tree & tree & bush & cloud & moon & sun & arch\_of\_triumph & big\_ben & castle \\
church & eiffel\_tower & leaning\_tower\_of\_pisa & moai\_stone & pyramids\_of\_giza & skyscraper & statue\_of\_liberty & stonehenge & sphinx & barn \\
bridge & fence & hospital & house & igloo & windmill & bench & fountain & fire hydrant & streetlight \\
traffic light & campfire & ferris\_wheel & roller\_coaster & lighthouse & angel & diamond & mermaid & patrick\_star & santa\_claus \\
skull & snowman & sponge\_bob & dragon & mona\_lisa & teddy bear & stop sign & jack o lantern & beach & rainbow \\
\end{tabular*}
\end{table*}



==> tbl/classificationcomparison/item.tex <==
\begin{table}[t]
\caption{Comparison of classification accuracy between human and CLIP-ViT-L/14 on \emph{CommonSketch}, \emph{TU Berlin}, \emph{QuickDraw}, \emph{SEVA}, and \emph{Pictogram} dataset. 
SEVA OOD denotes evaluation on SEVA classes that are out of distribution with respect to CommonSketch.}
\label{tab:jaeyoonclassification}
\centering
\scriptsize
\setlength{\tabcolsep}{4pt}
\begin{tabular}{l|ccccc}
\toprule
 & \makecell{\textbf{Common}\\\textbf{Sketch}} & \textbf{TU Berlin} & \textbf{QuickDraw} & \makecell{\textbf{SEVA}\\\textbf{OOD}} & \textbf{Pictogram} \\
\midrule
Human & 0.95 & 0.87 & 0.75 & 0.48 & 0.96 \\
CLIP-ViT-L/14 & 0.86 & 0.72 & 0.20 & 0.13 & 0.46\\
\bottomrule
\end{tabular}
\end{table}


==> tbl/cognitive_align/item.tex <==
\begin{table}[t]
\centering
\caption{Results on the \textit{CommonSketch} dataset for identifying a zero-shot classification model that best approximates human perception. We collect human assessments and run zero-shot classification on the same items, reporting Top-1 accuracy and correlations with human judgments (Spearman’s $\rho$, Kendall’s $\tau$, Pearson’s $r$; higher is better). The \textit{Human} row shows dashes because it is the reference rather than a predictive model.}
\small
\setlength{\tabcolsep}{6pt}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l c c c c@{}}
\toprule
\textbf{Model} & \textbf{Top1 Acc} & \textbf{Spearman's} & \textbf{Kendall's} & \textbf{Pearson's} \\
\midrule
Human    & -- & -- & -- & -- \\
\midrule
CLIP     &    &    &    &    \\
OpenCLIP &    &    &    &    \\
CoCa     &    &    &    &    \\
\bottomrule
\end{tabular*}
\end{table}

==> tbl/metric_explain/item.tex <==
\begin{table}[tbp]
\centering
\fontsize{9}{11}\selectfont
\setlength{\tabcolsep}{4pt}
\begin{tabular}{c|c|l}
\toprule
Metric Range & Interpretation & Description \\
\midrule
$\geq 1.0$ & Excellent abstraction & cognition exceeds information loss \\
$0.5$ – $1.0$ & Good abstraction & significant recovery despite some loss \\
$0.0$ – $0.5$ & Incomplete abstraction & high loss, partial recovery \\
$< 0.0$ & Cognitive confusion or failure & recognition lower than visible information \\
\bottomrule
\end{tabular}
\caption{Interpretation of Sketch Abstraction Metric values
}
\label{metric_explain}
\end{table}

==> tbl/three_correlation/item.tex <==
\begin{table}[t]
  \centering
  \scriptsize
  \caption{\textbf{Correlation of human evaluations with SEA score} from GPT-4o and Qwen.}
  \label{tab:cor_human_model}
  \begin{tabular}{l|cc}
    \toprule
    \textbf{Metric (VLM)} & \textbf{Spearman’s $\rho$} & \textbf{Pearson’s $r$} \\
    \midrule
    SEA (GPT-4o) & 0.457 & 0.564 \\
    SEA (Qwen2.5-VL)   & 0.501 & 0.582 \\
    \bottomrule
  \end{tabular}
\end{table}
